AutoRF: Learning 3D Object Radiance Fields from Single View Observations

We introduce AutoRF - a new approach for learning neural 3D object representations where each object in the training set is observed by only a single view. This setting is in stark contrast to the majority of existing works that leverage multiple views of the same object, employ explicit priors during training, or require pixel-perfect annotations. To address this challenging setting, we propose to learn a normalized, object-centric representation whose embedding describes and disentangles shape, appearance, and pose. Each encoding provides well-generalizable, compact information about the object of interest, which is decoded in a single-shot into a new target view, thus enabling novel view synthesis. We further improve the reconstruction quality by optimizing shape and appearance codes at test time by fitting the representation tightly to the input image. In a series of experiments, we show that our method generalizes well to unseen objects, even across different datasets of challenging real-world street scenes such as nuScenes, KITTI, and Mapillary Metropolis.

==> fig/fig_edit_color.tex <==
\begin{figure}[ht]

\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{cc}
    \centering
    \begin{minipage}{2.20\columnwidth}
        \includegraphics[width=.99\columnwidth]{fig/input2.PNG}
    \end{minipage} 
    & 
    \begin{minipage}{2.20\columnwidth}
        \includegraphics[width=.99\columnwidth]{fig/48.PNG}
    \end{minipage} \\
    \begin{minipage}{2.20\columnwidth}
        \includegraphics[width=.99\columnwidth]{fig/74.png}
    \end{minipage}
    &
    \begin{minipage}{2.20\columnwidth}
        \includegraphics[width=.99\columnwidth]{fig/97.png}
    \end{minipage}
\end{tabular}}
\caption{
    Color interpolation: starting from the properties of the objects in the input view (top-left), AutoRF is able to modify the properties of each object in the scene.
}
\label{fig:color_interp_supp}
\end{figure}

==> fig/fig_edit_scene.tex <==
\begin{figure}[ht]

\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{cc}
    \centering
    \begin{minipage}{2.20\columnwidth}
        \includegraphics[width=.99\columnwidth]{fig/input2.PNG}
    \end{minipage} 
    & 
    \begin{minipage}{2.20\columnwidth}
        \includegraphics[width=.99\columnwidth]{fig/261.PNG}
    \end{minipage} \\
    \begin{minipage}{2.20\columnwidth}
        \includegraphics[width=.99\columnwidth]{fig/310.png}
    \end{minipage}
    &
    \begin{minipage}{2.20\columnwidth}
        \includegraphics[width=.99\columnwidth]{fig/354.png}
    \end{minipage}
\end{tabular}}
\caption{
    Scene editing: starting from the objects in the input view (top-left), AutoRF is able to apply arbitrary modifications and also include novel objects. Results on an unseen image of the nuScenes dataset.
}
\label{fig:scene_editing_supp}
\end{figure}

==> fig/overview.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=.99\columnwidth]{example-image-golden}
\hfill
\includegraphics[width=.99\columnwidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Outline -- }
A figure summarizing the entire algorithm
}
\label{fig:overview}
\end{figure*}

==> fig/teaser.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Teaser -- }
Some nice summarizing image.
}
\label{fig:teaser}
\end{figure}

==> tab/results_nusc_val.tex <==
\begin{table}[]
\begin{tabular}{c|cccc}
nuScenes cars                      & PSNR ↑                    & SSIM ↑                    & LPIPS ↓                   & FID ↓                      \\ \hline
pixelNeRF                  & 18.25                     & 0.459                     & 0.236                     & 160.6                      \\
\multicolumn{1}{l|}{\Ours{} (no opt.) on train} & 18.58                     & \multicolumn{1}{l}{0.473} & 0.211                     & \textbf{84.14}             \\
\Ours{} on train                 & \textbf{18.95}            & \textbf{0.493}            & \textbf{0.210}            & 106.5                      \\
\multicolumn{1}{l|}{\Ours{} (no opt.) on test}  & \multicolumn{1}{l}{18.69} & \multicolumn{1}{l}{0.479} & \multicolumn{1}{l}{0.227} & \multicolumn{1}{l}{138.23} \\
\Ours{} on test                 & 18.94                     & 0.491                     & 0.223                     & 145.1                     
\end{tabular}
\label{tab:nusc_val_full}
\end{table}
